Graphs, spectral triples and Dirac zeta functions

To a finite, connected, unoriented graph of Betti-number g>=2 and valencies >=3 we associate a finitely summable, commutative spectral triple (in the sense of Connes), whose induced zeta functions encode the graph. This gives another example where non-commutative geometry provides a rigid framework for classification.

==> def.tex <==
\makeatletter
\newcommand{\bfm}[1]     {\mbox{\boldmath$#1$}}
\newcommand{\g}[1]       {\mathfrak#1}
\newcommand{\m}          {\mathfrak{m}}
\newcommand{\A}          {\mathcal{A}}
\newcommand{\ud}          {\mathrm{d}}
\newcommand{\p}          {\partial}
\newcommand{\C}          {\mathbb{C}}
\newcommand{\e}          {\textrm{ exp}}
\newcommand{\F}          {\mathcal{F}}
\newcommand{\G}          {\mathcal{G}}
\newcommand{\Hom}          {\mathop{\mathrm{Hom}} \nolimits}
\newcommand{\cok}          {\mathop{\mathrm{coker}} \nolimits}
\newcommand{\Tor}          {\mathop{\mathrm{Tor}} \nolimits}
\newcommand{\Ext}          {\mathop{\mathrm{Ext}} \nolimits}
\newcommand{\depth}          {\mathop{\mathrm{depth}} \nolimits}
\newcommand{\Fitt}          {\mathop{\mathrm{Fitt}} \nolimits}
\newcommand{\im}          {\mathop{\mathrm{im}} \nolimits}
\newcommand{\Depth}          {\mathop{\mathrm{depth}} \nolimits}
\newcommand{\Sym}          {\mathop{\mathrm{Sym}} \nolimits}
\newcommand{\Ann}          {\mathop{\mathrm{Ann}} \nolimits}
\newcommand{\pd}          {\mathop{\mathrm{pd}} \nolimits}
\newcommand{\I}          {\mathcal{I}}
\newcommand{\Ham}        {\mathbf{H}}
\newcommand{\tb}        {\mathcal{M}}
\newcommand{\Pic}          {\mathop{\mathrm{Pic}} \nolimits}
\newcommand{\N}          {\mathbb{N}}
\newcommand{\Nb}          {\mathcal{N}}
\newcommand{\ov}          {\overline}
\newcommand{\OX}          {\mathcal{O}_{X}}
\newcommand{\OY}          {\mathcal{O}_{Y}}
\newcommand{\Cliff}          {\mathop{\mathrm{Cliff}} \nolimits}
\newcommand{\OO}          {\mathcal{O}}
\newcommand{\Q}          {\mathbb{Q}}
\newcommand{\R}          {\mathbb{R}}
\newcommand{\PR}          {\mathbb{P}}
\newcommand{\K}          {\mathbb{K}}
\newcommand{\br}          {\buildrel}
\newcommand{\Sc}         {\mathcal{S}}
\newcommand{\Z}          {\mathbb{Z}}
\newcommand{\Lb}          {\mathcal{L}}
\newcommand{\reg}          {\mathop{\mathrm{reg}} \nolimits}
\newcommand{\lra}          {\longrightarrow}
\newcommand{\ra}          {\rightarrow}
\newcommand{\bea}          {\begin{eqnarray}}
\newcommand{\eea}          {\end{eqnarray}}


\newcommand{\ds}         {\displaystyle}
\newcommand{\scs}        {\scriptstyle}
\newcommand{\llp}        {\mbox{\rm\large (}}
\newcommand{\lrp}        {\mbox{\rm\large )}}
\newcommand{\Llp}        {\mbox{\rm\Large (}}
\newcommand{\Lrp}        {\mbox{\rm\Large )}}

\newenvironment{LPA}{\par\addvspace{\abovedisplayskip}%
\noindent\hfill$\displaystyle}{$\hfill\ignorespaces\unskip}

\newcommand{\ad}         {\mathop{\mathrm{ad}}         \nolimits}
\newcommand{\Ad}         {\mathop{\mathrm{Ad}}         \nolimits}
\newcommand{\Ai}         {\mathop{\mathrm{Ai}}         \nolimits}
\newcommand{\Anti}       {\mbox{A}}
\newcommand{\arccotan}   {\mathop{\mathrm{arccotan}}   \nolimits}
\newcommand{\arcsinh}    {\mathop{\mathrm{arcsinh}}    \nolimits}
\newcommand{\arctanh}    {\mathop{\mathrm{arctanh}}    \nolimits}
\newcommand{\Aut}        {\mathop{\mathrm{Aut}}        \nolimits}
\newcommand{\BAd}        {\mathop{\mathbf{Ad}}         \nolimits} % bf
\newcommand{\Beta}       {\mbox{B}}
\newcommand{\buitenmaat} {\mbox{outer measure}}
\newcommand{\cent}       {\mathop{\mathrm{center}}     \nolimits}
\newcommand{\comple}     {\mathop{\mathrm{c}}          \nolimits}
\newcommand{\Cl}         {\mathop{\mathrm{Cl}}         \nolimits}
\newcommand{\codim}      {\mathop{\mathrm{codim}}      \nolimits}
\newcommand{\conj}       {\mathop{\mathrm{conj}}       \nolimits}
\newcommand{\cotanh}     {\mathop{\mathrm{cotanh}}     \nolimits}
\newcommand{\curl}       {\mathop{\mathrm{curl}}       \nolimits}
\newcommand{\Der}        {\mathop{\mathrm{Der}}        \nolimits}
\newcommand{\diag}       {\mathop{\mathrm{diag}}       \nolimits}
\newcommand{\diameter}   {\mathop{\mathrm{diameter}}   \nolimits}
\newcommand{\divergentie}{\mathop{\mathrm{div}}        \nolimits}
\newcommand{\dom}        {\mathop{\mathrm{dom}}        \nolimits}
\newcommand{\End}        {\mathop{\mathrm{End}}        \nolimits}
\newcommand{\GL}         {\mathop{\mathbf{GL}}         \nolimits} % bf
\newcommand{\gr}         {\mathop{\mathrm{deg}}        \nolimits}
\newcommand{\grad}       {\mathop{\mathrm{grad}}       \nolimits}
\newcommand{\graphic}    {\mathop{\mathrm{graph}}      \nolimits}
\newcommand{\Her}        {\mbox{H}}
\newcommand{\hyp}        {\mathop{\mathrm{hyperarea}}  \nolimits}
\newcommand{\ima}        {\mathop{\mathrm{im}}         \nolimits}
\newcommand{\interior}   {\mathop{\mathrm{int}}        \nolimits}
\newcommand{\lengte}     {\mathop{\mathrm{length}}     \nolimits}
\newcommand{\Leb}        {\mathop{\,\raisebox{.04ex}{$\mathrm{L}$}}\nolimits}
\newcommand{\Li}         {\mathop{\mathrm{Li}}         \nolimits}
\newcommand{\Lie}        {\mathop{\mathrm{Lie}}        \nolimits}
\newcommand{\Lin}        {\mathop{\mathrm{Lin}}        \nolimits}
\newcommand{\Lo}         {\mathop{\mathbf{Lo}}         \nolimits} % bf
\newcommand{\M}          {\mathop{\mathrm{Mat}}        \nolimits}
\newcommand{\notsubset}  {\mbox{$\not\subset$}}
\newcommand{\opp}        {\mathop{\mathrm{area}}       \nolimits}
\newcommand{\Orth}       {\mbox{\textbf O}}
\newcommand{\Proj}       {\mbox{P}}
\newcommand{\qm}[1]      {\qquad\mbox{#1}\qquad}
\newcommand{\rank}       {\mathop{\mathrm{rank}}       \nolimits}
\newcommand{\Res}        {\mathop{\mathrm{Res}}        \nolimits}
\newcommand{\Resi}       {\mathop{\mathrm{Res}}                 }
\newcommand{\rk}         {\mathop{\mathrm{rk}}         \nolimits}
\newcommand{\rotatie}    {\mathop{\mathrm{curl}}       \nolimits}
\newcommand{\sgn}        {\mathop{\mathrm{sgn}}        \nolimits}
\newcommand{\sinlemn}    {\mathop{\mathrm{sl}}         \nolimits}
\newcommand{\slin}       {\mathop{\g{s}\g{l}}          \nolimits}
\newcommand{\SL}         {\mathop{\mathbf{SL}}         \nolimits} % bf
\newcommand{\SO}         {\mathop{\mathbf{SO}}         \nolimits} % bf
\def\Sp                  {\mathop{\mathbf{Sp}}         \nolimits} % bf
\newcommand{\Spin}       {\mathop{\mathbf{Spin}}       \nolimits} % bf
\newcommand{\SU}         {\mathop{\mathbf{SU}}         \nolimits} % bf
\newcommand{\su}         {\mathop{\g{s}\g{u}}          \nolimits}
\newcommand{\supp}       {\mathop{\mathrm{supp}}       \nolimits}
\newcommand{\Ti}         {\mathop{\mathrm{Ti}}         \nolimits}
\newcommand{\trace}      {\mathop{\mathrm{tr}}         \nolimits}
\newcommand{\U}          {\mathop{\mathrm{U}}          \nolimits}
\newcommand{\vol}        {\mathop{\mathrm{vol}}        \nolimits}
\newcommand{\Vp}         {\mathop{\mathrm{Vp}}         \nolimits}

\renewcommand{\Im}       {\mathop{\mathrm{Im}}         \nolimits}
\renewcommand{\Re}       {\mathop{\mathrm{Re}}         \nolimits}

%  DE VOLGENDE LENGTES ZIJN GEDEFINIEERD OM EXTRA RUIMTE TUSSEN RIJEN IN
%  ARRAY EN TABULAR ENVIRONMENTS TE KUNNEN MAKEN (GEBRUIK: ``\\[\...ARR]'').
%                    WE MAKEN GEBRUIK VAN ``\...ARR'' INDIEN:

\newlength{\extarr }  % IN BEIDE RIJEN GEEN SPECIALE DINGEN VOORKOMEN.
\newlength{\prtarr }  % IN 1 VAN DE 2 RIJEN \frac ed. VOORKOMEN.
\newlength{\dprtarr}  % IN BEIDE RIJEN \frac.
\newlength{\limarr }  % IN 1 VAN DE 2 RIJEN \lim, \sup, \inf, ETC.
\newlength{\sumarr }  % IN 1 VAN DE 2 RIJEN \sum, \prod, ETC.
\newlength{\intarr }  % IN 1 VAN DE 2 RIJEN \int.
\newlength{\matarr }  % IN 1 VAN DE 2 RIJEN EEN MATRIX, DETERMINANT.
\newlength{\dmatarr}  % IN BEIDE RIJEN EEN MATRIX.
\newlength{\ddetarr}  % IN BEIDE RIJEN EEN DETERMINANT.

% IN HET GEVAL DAT EEN VERGELIJKING UIT MEER DAN DRIE REGELS BESTAAT
% KAN MEN GEBRUIK MAKEN VAN HET QUOTE ENVIRONMENT OMDAT DEZE WEL TUSSEN REGELS
% KAN WORDEN AFGEBROKEN EN ZO DUS underfull \vbox KAN WORDEN VOORKOMEN.
% OM ENIGSZINS VERGELIJKBARE TUSSENRUIMTE TE KRIJGEN WORDEN DAARVOOR
% LENGTES \...QUO UIT \...ARR BEPAALD.

\newlength{\extquo }
\newlength{\prtquo }
\newlength{\dprtquo}
\newlength{\limquo }
\newlength{\sumquo }
\newlength{\intquo }
\newlength{\matquo }
\newlength{\dmatquo}
\newlength{\ddetquo}

\setlength{\extarr} { .2cm}
\setlength{\prtarr} { .3cm}
\setlength{\dprtarr}{ .5cm}
\setlength{\limarr} { .3cm}
\setlength{\sumarr} { .7cm}
\setlength{\intarr} { .7cm}
\setlength{\matarr} { .5cm}
\setlength{\dmatarr}{ .8cm}
\setlength{\ddetarr}{1.2cm}
\setlength{\extquo} {\extarr }
\setlength{\prtquo} {\prtarr }
\setlength{\dprtquo}{\dprtarr}
\setlength{\limquo} {\limarr }
\setlength{\sumquo} {\sumarr }
\setlength{\intquo} {\intarr }
\setlength{\matquo} {\matarr }
\setlength{\dmatquo}{\dmatarr}
\setlength{\ddetquo}{\ddetarr}

\addtolength{\extquo} {-.0 cm}
\addtolength{\prtquo} {-.0 cm}
\addtolength{\dprtquo}{-.25cm}
\addtolength{\limquo} {-.1 cm}
\addtolength{\sumquo} {-.4 cm}
\addtolength{\intquo} {-.2 cm}
\addtolength{\matquo} {-.3 cm}
\addtolength{\dmatquo}{-.3 cm}
\addtolength{\ddetquo}{-.35cm}

\swapnumbers

\newtheorem{Conj}[subsection]{Conjecture}
\newtheorem{Coro}[subsection]{Corollary}
\newtheorem{Lemm}[subsection]{Lemma}
\newtheorem{Prop}[subsection]{Proposition}
\newtheorem{Theo}[subsection]{Theorem}


%\theoremstyle{Remark}

\theoremstyle{definition}
\newtheorem{Tex}[subsection]{}
\newtheorem{Defi}[subsection]{Definition}
\newtheorem{Voor}[subsection]{Example}
\newtheorem{Rem}[subsection]{Remark}


\newenvironment{Proof}      {\medskip\noindent {\bf Proof.}}{\unskip\nobreak\hfill\ding{111}\par\medskip}
\newenvironment{Conjecture} [2]{\bigskip\begin{Conj} #1 \label{Conjecture  #2}   }{\end{Conj}\medskip}
\newenvironment{Corollary}  [2]{\bigskip\begin{Coro} #1 \label{Corollary   #2}   }{\end{Coro}\medskip}
\newenvironment{Definition} [1]{\bigskip\begin{Defi}    \label{Definition  #1}\rm}{\unskip\nobreak\hfill\ding{109}\end{Defi}\medskip} \newenvironment{Lemma}      [2]{\bigskip\begin{Lemm} #1 \label{Lemma       #2}   }{\end{Lemm}\medskip}
\newenvironment{Proposition}[2]{\bigskip\begin{Prop} #1 \label{Proposition #2}   }{\end{Prop}\medskip}
\newenvironment{Theorem}    [2]{\bigskip\begin{Theo} #1 \label{Theorem     #2}   }{\end{Theo}\medskip}
\newenvironment{Voorbeeld}  [2]{\bigskip\begin{Voor} #2 \label{Voorbeeld   #1}\rm}{\unskip\nobreak\hfill\ding{80}\end{Voor}\medskip}

\newcounter{vrghfdstuk}     [section]
\newtheorem{Vrg}{Exercise}  [vrghfdstuk]
\newenvironment{Vraagstuk}  [2]{\smallskip\begin{Vrg}#2  \label{Vraagstuk #1} \rm}{\end{Vrg}\smallskip}

\renewcommand{\topfraction}   {1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}  {0}

\makeatletter
\def\dum{This is an example of simple text.\par}

\newcount\checkxx \checkxx=0
\def\simpletext#1{\loop
    \ifnum\checkxx<#1
        \the\checkxx. \dum\advance\checkxx\@ne
    \repeat
}
\makeatother

%\setlength\textheight{39\baselineskip}
%\addtolength\textheight{\topskip}
%\textwidth26pc
%\topmargin 29pt
%\headheight13pt
%\footskip26pt
%\topskip10pt

\newenvironment{LPB}[1]{\par%
\addvspace{\abovedisplayskip}%
$#1}{$\par\vspace*{-18pt}}

\let\LP\LPA
\let\endLP\endLPA


\def\contentsname{Table of Contents}

\gdef\ps@headings{%
      \let\@oddfoot\@empty\let\@evenfoot\@empty
      \def\@evenhead{\thepage\hfil\slshape\leftmark}%
      \def\@oddhead{{\slshape\rightmark}\hfil\thepage}%
      \let\@mkboth\markboth
    \def\chaptermark##1{%
      \markboth {\MakeUppercase{%
        \ifnum \c@secnumdepth >\m@ne
          \if@mainmatter
            \@chapapp\ \thechapter. SURESH\ %
          \fi
        \fi
        ##1}}{}}%
    \def\sectionmark##1{%
      \markright {\MakeUppercase{%
        \ifnum \c@secnumdepth >\z@
          \thesection. SURESH\ %
        \fi
        ##1}}}}
\makeatother

% VERDERE INFORMATIE BENODIGD VOOR DE INDEX EN DE LIJST VAN NOTATIES.
% DE VOLGENDE COMMANDOS ZIJN NODIG OM DE INDEX MET GETOONDE INHOUD TE MAKEN

%\addcontentsline{toc}{section}{Index}
%\begin{theindex}
%\small{
%\item {\large \bf A}
%\item \hspace{.2cm} Afbeelding, $C^{\infty}$- van vari\"{e}teiten 255
%\item \hspace{.2cm} Afsluiting   87
%\item \hspace{.2cm} ---, in deelvari\"{e}teit 140
%\item \hspace{.2cm} Amplitude 128
%\vspace{2.5ex}
%\item {\large \bf B}
%\item \hspace{.2cm} Beginwaardeprobleem, voor golfvergelijking 301
%\item \hspace{.2cm} ---, voor warmtevergelijking 128
%\vspace{2.5ex}
%\item {\large \bf Y}
%\item \hspace{.2cm} Young, ongelijkheid van 233
%}
%\end{theindex}

% De programmatuur voor het sorteren van de indexfiles is in een algemene
% directory gezet.
% Men kan deze aanroepen door het geven van het commando: index
% Daarna vraagt de computer om de naam van de idx-file zonder de extensie .idx
% De output heeft voorlopig de extensie .out
% Zelf moet men toevoegen boven aan de file de opdracht:
% \addcontentsline{toc}{section}{Index}
% Voorts moet men nog komma's op geeigende plaatsen toevoegen.

% DE VOLGENDE COMMANDOS ZIJN NODIG OM DE LIJST MET NOTATIES TE MAKEN
% LET OP DE AFSTANDEN

%\chapter*{Notaties}
%\markboth{}{}
%\addcontentsline{toc}{section}{Notaties}
%\begin{tabular}{lp{11cm}r}
%$\times$                          & Vectorieel uitproduct & 57 \\
%$\Delta$                          & Laplace-operator & 178 \\
%\end{tabular}

% De inputfile analc.glo moet worden opgeschoond met de teksteditor,
% en kan worden gesorteerd met de sorteerroutine sort uit UNIX.
% Het beste is het om eerst analc.glo te copieren naar een hulpfile hulp.tex
% Dan het commando: cat hulp.tex | sort > not.tex
% Het eindresultaat is een gesorteerde file not.tex

% END OF FILE 

